Social Distancing via Social Scheduling

Motivated by the need of {\em social distancing} during a pandemic, we consider an approach to schedule the visitors of a facility (e.g., a general store). Our algorithms take input from the citizens and schedule the store's discrete time-slots based on their importance to visit the facility. Naturally, the formulation applies to several similar problems. We consider {\em indivisible} job requests that take single or multiple slots to complete. The salient properties of our approach are: it (a)~ensures social distancing by ensuring a maximum population in a given time-slot at the facility, (b)~aims to prioritize individuals based on the importance of the jobs, (c)~maintains truthfulness of the reported importance by adding a {\em cooling-off} period after their allocated time-slot, during which the individual cannot re-access the same facility, (d)~guarantees voluntary participation of the citizens, and yet (e)~is computationally tractable. The mechanisms we propose are prior-free. We show that the problem becomes NP-complete for indivisible multi-slot demands, and provide a polynomial-time mechanism that is truthful, individually rational, and approximately optimal. Experiments with data collected from a store show that visitors with more important (single-slot) jobs are allocated more preferred slots, which comes at the cost of a longer cooling-off period and significantly reduces social congestion. For the multi-slot jobs, our mechanism yields reasonable approximation while reducing the computation time significantly.

==> app.tex <==
\pagebreak
\section*{Appendix}

\section{Proof of \Cref{thm:relax}}



\section{Proof of \Cref{lem:equivalence}}



\section{Proof of \Cref{lem:MUCA_reduction}}



\section{Proof of \Cref{lem:alg2_validity}}

% 


\section{Proof of \Cref{lem:alg2IC}}



\section{Proof of \Cref{thm:dsic}}\label{APP_DSIC}


\section{Proof of \Cref{thm:ir}}\label{APP_IR}



% \section{Proof of \Cref{thm:NPc}}\label{NPC_proof}
% % The LP relaxation of the IP~\ref{eqn:MULTIALLOC_IP} is identical to LP~\ref{eqn:LP} without the first set of constraints and hence, the constraint matrix of new LP is also TU. Therefore, the new LP also gives integral solutions which is an optimal solution to the IP~\ref{eqn:MULTIALLOC_IP}.
% We denote the decision version of \multi\ with the same name, which is defined as follows:
% \begin{quote} % looks better
% Given $(N,M,V,L,k,\beta)$, is there an allocation $\AA$ such that $\sum_{i \in N} \sum_{p \in M,\  j \leqslant p+l_i-1} \aaa_{ip} \leqslant k \ \forall j \in M, \ \sum_{j \in M} \aaa_{ij} \leqslant 1\  \forall i \in N$, and $\sum_{i \in N} \sum_{j \in M}  v_{ij}\ \aaa_{ij}\geqslant \beta$ where $\beta\in\mathbb{R}$.
% \end{quote}
% \begin{proof}
% % \par $P1$ is a decision problem for the \multi\  implies that, if there exists a polynomial algorithm that solves the $P1$, then one can find the maximum value for the job allocation problem in polynomial time by applying this algorithm iteratively while increasing the value of $b$. On the other hand, if an algorithm finds the optimal value of the job allocation problem in polynomial time, then $P1$ can be solved in polynomial time by comparing the solution output's value by this algorithm the value of $b$. \\
% To prove that \multi\  is in $NP$, we have to show that, ``given an allocation $\AA$, one can verify in polynomial time that $\AA$ is a valid solution for \multi.'' The verification will need to solve and check the $(m+n+mn)$ linear constraints and the objective function of \Cref{eqn:MULTIALLOC_IP}. Therefore, the computation of the value of objective function and comparison with $\beta$ is doable in $O(mn)$ time. Hence, \multi\  is in NP.

% Next, we show that ``every problem in NP is reducible to \multi\  in polynomial time". To prove this, we take a sub-problem of \multi\, and in \Cref{lem:subset_NPC}, we prove that the sub-problem is NP-complete, which implies ``every problem in NP is reducible to a sub-problem of \multi\ in polynomial time."

% \begin{lemma}\label{lem:subset_NPC}
% There exist an NP-complete sub-problem of \multi.
% \end{lemma}
% \begin{proof} Consider the subset of \multi\ such that the valuation of every agent ($v_i$) is independent of the starting point of her job during the period. We call this sub-problem as \textsc{sub\_multi}. In this proof, we represent the valuation as a tuple $\VV$ of length $n$. Let for \textsc{sub\_multi} $k=1$. 
% % Now, each unit of the slot capacity ($k$) can be thought of a counter. Each counter processes one job until it is complete. The set of counters is denoted by $K=\{ 1,2,\dots,k \}$. We denote the set of all \textit{job-to-counter} allocations by $\mathcal{X}$. An allocation $X\in\mathcal{X}$, is a matrix $[x_{ic}]$ such that:
% % \begin{equation*}
% % x_{ic}=
% %     \begin{cases}
% %     1, & \text{if agent $i$'s job is allocated to counter $c$}\\
% %     0, & \text{otherwise}
% %     \end{cases}
% % \end{equation*}
% Mathematically, \textsc{sub\_multi} is given by the following integer program (IP).

% \begin{align}
% \label{eqn:SUB_MULTIALLOC_IP}
%  \begin{split}
%       \argmax_{A} & \sum_{i \in N} \sum_{j \in M}  v_{i}\ \aaa_{ij} \\
%      \text{s.t. } & \sum\limits_{i \in N} \sum\limits_{\substack{p \in M \\ j \leqslant p+l_i-1}} \aaa_{ip} \leqslant 1, \forall j \in M \\ &
%      \sum_{j \in M} \aaa_{ij} \leqslant 1, \forall i \in N, \\
%      &
%      \aaa_{ij}\in \{ 0,1\}, \forall i \in N, \forall j \in M
%  \end{split}
% \end{align}

% We denote the decision version of \textsc{sub\_multi} with the same name, which is defined as follows:
% \begin{quote}
% Given $(N,M,\VV,L,k,\beta)$, is there an allocation $X$ such that $\sum_{i \in N} \sum_{p \in M,\  j \leqslant p+l_i-1} \aaa_{ip} \leqslant 1\  \forall j \in M$, $\sum_{j \in M} \aaa_{ij} \leqslant 1\  \forall i \in N$, $\aaa_{ij}\in \{ 0,1\}$, and $\sum_{i \in N} \sum_{j \in M}  v_{i}\ \aaa_{ij} \geqslant \beta$ where $\beta\in\mathbb{R}$.
% \end{quote}
% \textit{Proof for NP-completeness:} It is easy to see that, given an allocation, the verification will need to solve and check the $(m+n+mn)$ linear constraints, and solve the objective function. Therefore, the computation of the value of objective function and comparison with $\beta$ is doable in polynomial $(O(mn))$ time. Hence, \textsc{sub\_multi} is in NP.

% Next we have to show that, ``every problem in NP is reducible to \textsc{sub\_multi} in polynomial time." To prove this, we select the classical \textsc{knapsack problem}, which is NP-complete and  show that it is reducible to \textsc{sub\_multi}. The \textsc{knapsack problem} is as follows: given a set of items $I=\{1,2,\dots,n\}$, their weights $W=(w_1,w_2,\dots,w_n)$, profits $P=(p_1,p_2,\dots,p_n)$ and a knapsack of capacity $\kappa$, find a subset $Y$ of items from $I$ such that the total profit of the selected items is maximum, and the total weights of the selected items does not exceed $\kappa$. Let $y$ be a vector such that, $y_i=1$ if $i \in Y$, and $y_i=0$ otherwise. The decision version of the knapsack problem is: ``Given $(I,P,W,\kappa,\beta')$, is there a vector $y$ such that $\sum_{i\in I} y_i\ w_i \leqslant \kappa$, and for which $\sum_{i\in I} p_i y_i \geq$ $\beta'$ where $\beta' \in \mathbb{R}$."

% Consider the following reduction: let the set of items $I$ to be the set of agents $N$, the items' profits $P$ to be the value of agents' jobs in $\VV$, the items' weights $W$ to be the length of the jobs in $L$, and the capacity of the knapsack $\kappa$ to be the number of slots $m$. The {\sc knapsack problem}$(I,P,W,\kappa,\beta')$ is then reduced (in polynomial time) to \textsc{sub\_multi}$(I, \{1, 2, \ldots, \kappa \}, P, W, \beta')$. And the solution $y$ of \textsc{knapsack problem} can be constructed from the solution $\AA$ of \textsc{sub\_multi} such that, $y_i=1$ for $i \in I$, if $\sum_{j\in M} \aaa_{i}=1$ for $i \in N$, else $y_i=0$.
% \end{proof}
% As \multi\ is verifiable in polynomial time, from \Cref{lem:subset_NPC} we conclude that \multi\ is NP-complete.  
% \end{proof}


% % \section{Reduction of \multi\  to \MUCA}





\section{Restated results from \cite{bartal2003incentive}} \label{sec:Lemmata_bartal}

\section{Additional Experimental Results}



==> model_theory.tex <==
\section{Basic Problem Setup}
\label{sec:setup}

Define $N \coloneqq \{1, \ldots, n\}$ to be the set of agents that are trying to access a facility ${\cal F}$. Time is divided into {\em periods}, and each period is further divided into {\em slots}. The set of slots is denoted by $M \coloneqq \{1, \ldots, m\}$. Every slot has a maximum capacity of $k$, which is decided by the social distancing norm of the region and the size of the facility. A {\em central planner} (e.g., an AI app) allocates these slots to the agents maintaining the capacity constraint. Every agent has a preference over the slots which is represented by a real number against each slot. For instance, the preference (we will call this the agent's {\em valuation}) of agent $i$ for slot $j$ is denoted by $v_{ij} \in \mathbb{R}_{\geqslant 0}$, which is interpreted as if slot $j$ is allotted to $i$, then $i$ is willing to wait for $v_{ij}$ time periods before requesting another access to the facility.\footnote{The valuation $v_{ij}$ need not be integral. In practice, the facility will be frozen for that duration of time in the booking app.} Thus the valuation implicitly reflects the importance to visit the facility for that agent. 
% An example framework for such importance representation could be to assign finite levels of importance -- \texttt{urgent, medium, not-urgent} -- and assign fixed numbers for them. 
The valuation vector of $i$ is represented by $v_i \in \mathbb{R}_{\geqslant 0}^m$.
% 
In this paper, we consider different facilities independently.
The joint facility slot allocation problem can be modeled as a similar problem with the additional constraint that the same slot cannot be allocated to the same agent at different facilities. We leave the detailed analysis for it as a future work.

The planner decides the allocation which can be represented as a matrix $A = [a_{ij}]$, where $a_{ij} = 1$, if agent $i$ is allotted slot $j$, and zero otherwise. We assume that every agent can be assigned at most one slot in a period. We denote the slot assigned to $i$ by $a_i^*$. The planner also decides a delay $d = (d_i, i \in N)$ for each agent before which they cannot make another request to the system. We assume that every agent wants a more valued slot to be assigned to her and also wants to wait less. Therefore, the net payoff of an agent is assumed to follow a standard {\em quasi-linear form}~\cite{SL08}
\begin{equation}
    \label{eq:utility}
    u_i((A,d), v_i) = v_i(A) - d_i, \text{ where } v_i(A) = v_{i a_i^*}.
\end{equation}
Denote the set of all allocations by ${\cal A}$ and $d_i \in \mathbb{R}, \forall i \in N$. The planner does not know the valuations (or urgencies) of the agents. Therefore he needs the agents to report their valuations and decide the allocation and the delay. This leaves the opportunity for an agent to misrepresent her true valuation, e.g., an agent can report a \texttt{not-urgent} valuation as \texttt{urgent} for a prioritized scheduling. To distinguish, we use $v_{ij}$ for the true valuation and $\hat{v}_{ij}$ for reported valuations. We will use the shorthand $v = (v_i)_{i \in N}$ to denote the true valuation profile represented as an $m \times n$ real matrix, and $\hat{v}$ to denote the reported valuation profile. The notation $v_{-i}$ denotes the valuation profile of the agents except $i$.
% 
The decision problem of the planner is therefore formally captured by the following function.
\begin{definition}[Social Scheduling Function (SSF)]
 A {\em social scheduling function (SSF)} is a mapping $f : \mathbb{R}^{m \times n} \to {\cal A} \times \mathbb{R}^n$ that maps the reported valuations to an allocation and delay for every agent. Hence, $f(\hat{v}) = (A(\hat{v}), d(\hat{v}))$, where $A$ is the allocation and $d$ is the delay function.\footnote{We overload the notation $A$ and $d$ to denote both functions and values of those functions, since their use will be clear from the context.}
\end{definition}



% \sn{need to say something more}

\section{Preliminary Definitions}
\label{sec:desiderata}

In this section, we formally define a few desirable properties that a social scheduling algorithm should satisfy. The properties address the issues of prioritization, truthfulness, voluntary participation, and computational complexity.

The first property ensures that the allocation is {\em efficient} in each period, i.e., it maximizes the sum of the valuations of all the agents. As an effect, every slot will be allocated to an agent who values it the most, breaking ties arbitrarily.
\begin{definition}[Efficient Per Period (EPP)]
 \label{def:efficiency}
 An SSF $f$ is {\em efficient per period (EPP)} if at every period, it chooses an allocation $A^*$ that maximizes the sum of the valuations of all the agents. Formally, if $f(\cdot) = (A^*(\cdot), d(\cdot))$, then
 \begin{equation}
     \label{eq:efficient}
     A^*(v) \in \argmax_{A \in {\cal A}} \sum_{i \in N} \sum_{j \in M} v_{ij} a_{ij}.
 \end{equation}
\end{definition}

However, since the planner can only access the reported values $\hat{v}_i$'s which can be different from the true $v_i$'s, it is necessary that the reported values are indeed the true values. The following property ensures that the robots are incentivized to `truthfully' reveal these information.
\begin{definition}[Per Period Dominant Strategy Truthful]
 \label{def:non-manipulability}
 An SSF $f(\cdot) = (A(\cdot), d(\cdot))$ is {\em truthful in dominant strategies per period} if for every $v_i, \hat{v}_i, \hat{v}_{-i}$, and $i \in N$
  \begin{align*}
   \lefteqn{ v_i(A(v_i, \hat{v}_{-i})) - d_i(v_i, \hat{v}_{-i})} \\
   \quad &\geqslant v_i(A(\hat{v}_i, \hat{v}_{-i})) - d_i(\hat{v}_i, \hat{v}_{-i}).
  \end{align*}
\end{definition}
The inequality above shows that if the true value of agent $i$ is $v_i$, the allocation and delay resulting from reporting it `truthfully' maximizes her payoff {\em irrespective of the reports of the other robots}.

\begin{definition}[Individual Rationality]
 \label{def:ir}
 An SSF $f(\cdot) = (A(\cdot), d(\cdot))$ is {\em individually rational} if for every $v$, and $i \in N$
  \begin{align*}
   v_i(A(v)) - d_i(v) &\geqslant 0.
  \end{align*}
\end{definition}
Individual rationality ensures that it is always weakly beneficial for every rational agent to participate in such a mechanism.

In large facilities, the number and capacities of the slots are large, leading to an exponential increase in the size of the set ${\cal A}$. This largeness of ${\cal A}$ makes it challenging to find a solution quickly. There are problems for which a quick method of solving them is not known yet. Still, a given solution can be \textit{verified} quickly in time polynomial of the input size, which means that the given solution's validity can be tested quickly. The complexity class of such problems is known as \textit{NP (nondeterministic polynomial)}. We consider the NP-complete class of problems which is defined as follows.
\begin{definition}[NP-complete]
A decision problem $Q$ is NP-complete if:
\begin{enumerate}
    \item $Q $ is in NP (class of all decision problems verifiable in	polynomial time), and
    \item Every problem in NP is reducible to $Q$ in polynomial time.
\end{enumerate}
\end{definition}
We will show that the slot allocation problem in a certain setting belongs to this class.

In a practical setting, where the allocations and delays need to be decided before every period, it is desirable to have an SSF that is computable in a time polynomial in $n$ and $m$ so that it finishes the computation in a time negligible to the time duration of the period. We consider algorithms that are {\em strongly polynomial}. Strongly polynomial algorithms are defined by their arithmetic model of computation. The basic arithmetic operations (addition, subtraction, multiplication, division, and comparison) take a unit time step to perform, regardless of the sizes of the operands. 

% [refer to the wikipedia article: https://en.wikipedia.org/wiki/Time_complexity#Strongly_and_weakly_polynomial_time]

\begin{definition}[Strongly Polynomial]
 \label{def:strong-poly}
    An algorithm runs in {\em strongly polynomial time} if \citep{grotschel1993complexity}
    \begin{itemize}
        \item the number of operations in the arithmetic model of computation is bounded by a polynomial in the number of operands in the input instance; and
        \item the space used by the algorithm is bounded by a polynomial in the size of the input.
    \end{itemize}
\end{definition}



% \sn{need to say a few words}


\section{Periodic Mechanisms}
\label{sec:online}

We consider mechanisms that run at every period of this social scheduling problem. The agents report their valuations in the beginning of every period. The planner decides the schedules and delays.\footnote{For mechanisms that consider the finite or infinite horizon of such allocation problems \citep[e.g.]{bergemann-valimaki10dynamic-pivot}, (a)~the designer needs to know the transition probabilities, (b)~solution concepts are weaker, and (c)~are computationally expensive. These factors made us restrict our attention to periodic mechanisms.}

% \footnote{In a practical implementation, the decision might be taken one or two periods before since that provides the agents some time to be prepared.}

In our setting, the agents have the opportunity to overstate their urgencies to get a better slot allotted to them. This is precisely where our approach using the ideas of mechanism design \citep{borgers2015introduction} is useful. 

 In a setting where the agents' valuations are private, if the mechanism has no additional tool (e.g., delays in time in our context) to penalize overstating, only {\em dictatorial} mechanisms (where a pre-selected agent's favorite outcome is selected always) are truthful \citep{Gib73,Sat75}. This negative result holds irrespective of whether agents' preferences are {\em ordinal} (representable as an order relation over the outcomes) or {\em cardinal} (agents have a real number to represent the intensity of the preference). Note that in our setup, the agents' preferences are cardinal.
 A complementary analysis by \citet[Thm 7.2]{Roberts79} shows that a dictatorship result reappears under certain mild conditions in a {\em quasi-linear} setting (which is our current setting), unless transfers (of utility) are allowed. 
%  Transfers, in these settings, is used as a means of transferring value from an agent to another, and it is shown to help by unraveling the true values of the agents. 
 In this paper, we use delay as a surrogate for transferable utility among the agents to ensure truthful value revelation at every period. 
 
We are now in a position to present the proposed mechanism \mech\ (\mechfull).

\begin{algorithm}[h!]
 \caption{\mech\ in every period}
 \begin{algorithmic}[1]
   \STATE {\bf Input:} for every agent $i \in N$, the value $\hat{v}_i$
      \STATE compute $A^*(\hat{v})$ (\Cref{eqn:LP}) as the allocation \label{alg:allocation-step}
      \STATE charge a delay $d_i(\hat{v})$ (\Cref{eqn:payment}) to every $i \in N$ for which they cannot access the scheduling mechanism again
    \STATE {\bf Output:} $A^*(\hat{v})$ and $d(\hat{v})$
  \end{algorithmic}
 \label{algo:mechanism}
 \end{algorithm}
 
\paragraph{Description of \mech}

The SSF needs to decide on the allocation $A$ and the delay $d$. The actual allocation that satisfies EPP is given by the following integer program (IP).
\begin{align}
 \label{eqn:IP}
 \begin{split}
     \argmax_{A} & \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij} \\
     \text{s.t. } & \sum_{j \in M} a_{ij} \leqslant 1, \ \forall i \in N, \\
     & \sum_{i \in N} a_{ij} \leqslant k, \ \forall j \in M, \\
     & a_{ij} \in \{0, 1\}, \ \forall i \in N, j \in M.
 \end{split}
\end{align}
However, IPs are NP-complete in general. Therefore, \mech\ computes the LP relaxation of the above problem, given as follows.
\begin{align}
 \label{eqn:LP}
 \begin{split}
     \argmax_{A} & \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij} \\
     \text{s.t. } & \sum_{j \in M} a_{ij} \leqslant 1, \ \forall i \in N, \\
     & \sum_{i \in N} a_{ij} \leqslant k, \ \forall j \in M, \\
     & a_{ij} \geqslant 0, \ \forall i \in N, j \in M.
 \end{split}
\end{align}
We will show that this is without loss of optimality, since the solution to LP~\ref{eqn:LP} will always be integral and will coincide with the solution of IP~\ref{eqn:IP}. 

The delay of agents are computed via the standard Vickery-Clarke-Groves (VCG) rule \cite{Vick61,Clar71,Grov73}. Denote the optimal allocation of LP~\ref{eqn:LP} by $A^*(v)$. Also, denote the allocation given by LP~\ref{eqn:LP} when agent $i$ is removed from the system by $A^*_{-i}(v_{-i})$.
% 
For agent $i$, the delay is given by,
\begin{align}
\label{eqn:payment}
\begin{split}
    d_i &:= \sum_{\ell \in N \setminus \{i\}} v_\ell(A^*_{-i}) - \sum_{\ell \in N \setminus \{i\}}  v_\ell(A^*). 
\end{split}
\end{align}
The mechanism in every period is described in \Cref{algo:mechanism}.

Note that the allocation is different from that of a sorted importance sequential dictator, i.e., where the agents are sorted based on their importance and asked to pick their favorite slots in that order. For example, consider two agents A and B, and two slots of capacity one. Valuations are (51, 50) and (50, 0) respectively for A and B respectively for the two slots -- sequential dictator would allocate slot 1 to A and 2 to B, while the socially optimal is to allocate slots 2 and 1 to A and B respectively, which is allocated by \mech.

\section{Theoretical guarantees}
\label{sec:theory}


Our first result shows that \mech\ ensures proper prioritization of the agents and reveals their importance truthfully.
\begin{theorem}
\label{thm:dsic}
 \mech\ is per period dominant strategy truthful.
\end{theorem}


\shortversion{\noindent This proof of per period dominant strategy truthful is a standard extension of the proof for Vickery-Clarke-Groves (VCG) mechanism \cite{Vick61,Clar71,Grov73} and is available in the supplemental material.
}

\longversion{
\begin{proof}
 This proof is a standard exercise in the line of the proof for Vickery-Clarke-Groves (VCG) mechanism \cite{Vick61,Clar71,Grov73}. \mech\ follows the VCG allocation and payment locally at every intersection calculated by the LIM. Hence, the payoff of robot $i$ at intersection $k$ is given by (for brevity of notation, we hide the time argument in every function and write $a_k^*$ as $a_k^*(v_i, v_{-i})$)
% \begin{gather}
 \begin{align*}
   \lefteqn{ \val_i(a_k^*(v_i, \hat{v}_{-i}), v_i) - p_i(v_i, \hat{v}_{-i})} \\
   &= \sum_{j \in N_k}  \val_j(a_k^*(v_i, \hat{v}_{-i}), \hat{v}_j) - \sum_{j \in N_k \setminus \{i\}} \val_j(a_k^{*,N_k \setminus \{i\}}, \hat{v}_j) \\
   &\geqslant \sum_{j \in N_k}  \val_j(a_k^*(\hat{v}_i, \hat{v}_{-i}), \hat{v}_j) - \sum_{j \in N_k \setminus \{i\}} \val_j(a_k^{*,N_k \setminus \{i\}}, \hat{v}_j) \\
   &= \val_i(a_k^*(\hat{v}_i, \hat{v}_{-i}), v_i) - p_i(\hat{v}_i, \hat{v}_{-i}).
  \end{align*}
% \end{gather}
The first equality is obtained by writing and reorganizing the expression for $p_i$. The inequality holds since by definition $\sum_{j \in N_k}  \val_j(a_k^*(v_i, \hat{v}_{-i}), \hat{v}_j) \geqslant \sum_{j \in N_k}  \val_j(a_k, \hat{v}_j)$ for every $a_k$; in particular, we chose $a_k^*(\hat{v}_i, \hat{v}_{-i})$. The last equality is obtained by reorganizing the expressions again.
\end{proof}
}

The next result ensures that the agents are incentivized to voluntarily participate in \mech.
\begin{theorem}
 \label{thm:ir}
 \mech\ is individually rational for every agent.
\end{theorem}

\begin{proof}
 Consider agent $i$. The utility of $i$ under \mech\ is given by
 \begin{align*}
     \lefteqn{ v_i(A^*(v)) - d_i(v) } \\
     &= v_i(A^*) - \left( \sum_{\ell \in N \setminus \{i\}} v_\ell(A^*_{-i}) - \sum_{\ell \in N \setminus \{i\}}  v_\ell(A^*) \right) \\
     &= \left( \sum_{\ell \in N}  v_\ell(A^*) - \sum_{\ell \in N} v_\ell(A^*_{-i}) \right) + v_i(A^*_{-i}) \geqslant 0
 \end{align*}
 The second equality holds by reorganizing the terms and by adding and subtracting $v_i(A^*_{-i})$. Note that the difference term in the parentheses in the last expression is always non-negative since $A^*$ is the optimal allocation for all allocations. In particular, $A^*_{-i}$ is also a feasible allocation when agent $i$ is present. The term $v_i(A^*_{-i})$ is zero. Hence the inequality follows.
\end{proof}

The next few results show that even if the allocation problem of IP~\ref{eqn:IP} falls in a computationally intractable class, its special structure can be used to find a tractable solution.
\begin{theorem}
 \label{thm:relax}
 The allocation of \mech\ given by LP~\ref{eqn:LP} always gives integral solutions.
\end{theorem}

\begin{proof}
 Consider the vector $x^\top = (a_{11}, \ldots, a_{1m}, \ldots, a_{n1}, \ldots, a_{nm})$, i.e., the rows of $A$ linearized as a vector. We can write the constraints of LP~\ref{eqn:LP} in using a $(n+m) \times nm$ constraint matrix, s.t.,
 \[
 \left ( 
 \begin{array}{ccccccccc}
     1 & \ldots & 1 & 0 & \ldots & 0 & 0 & \ldots & 0 \\
     0 & \ldots & 0 & 1 & \ldots & 1 & 0 & \ldots & 0 \\
     &&&&\ldots&&&& \\
     1 & \ldots & 0 & 1 & \ldots & 0 & 1 & \ldots & 0 \\
     0 & 1 & \ldots & 0 & 1 & \ldots & 0 & 1 & 0 \\
     &&&&\ldots&&&&
 \end{array}
 \right ) x \leqslant \left ( \begin{array}{c}
     1 \\
      \vdots \\
      k \\
      \vdots
 \end{array}\right )\]
 Denote the matrix on the LHS by $C$. The first $n$ and the next $m$ rows correspond to the first and second set of constraints of LP~\ref{eqn:LP} respectively. We show that $C$ is totally unimodular (TU), which is sufficient to conclude that LP~\ref{eqn:LP} has integral solutions.
 We use the Ghouila-Houri characterization \cite{camion1965characterization} to prove that $C$ is TU. According to this characterization, a $p \times q$ matrix $C$ is TU if and only if each set $R \subseteq \{ 1,2, \cdots, p\}$ can be partitioned into two sets $R_1$ and $R_2$, such that, $\sum\limits_{i \in R_{1}} a_{ij} - \sum\limits_{i \in R_{2}} a_{ij} \in \{ 1,0,-1\}$, for $j= 1,2,\cdots,q$. Note that, in $C$ every column has two 1's, one in the first $n$ rows and one in the next $m$ rows. Pick any subset $R$ of the rows, construct the $R_1$ to be the rows that come from the first $n$ rows, and $R_2$ to be the rows that come from the last $m$ rows (one of these partitions can be empty). Clearly, the difference in each column of the rows $R$ will lie in $\{1,0,-1\}$. Hence proved.
\end{proof}

The result above shows that the optimal solution of LP~\ref{eqn:LP} is an optimal solution of IP~\ref{eqn:IP}. Hence, the mechanism is indeed doing an efficient allocation which can be summarized in the following corollary.
\begin{corollary}
\label{cor:efficient}
 \mech\ is EPP.
\end{corollary}

\Cref{thm:relax} shows that the solution to the LP relaxation of the allocation problem is without loss of optimality. LPs are known to be polynomially computable. However, in general it can be weakly polynomial, i.e., the space used by the algorithm may not be bounded by a polynomial in the size of the input. The forthcoming results show that the solutions of allocation and delays of \mech\ are strongly polynomial (\Cref{def:strong-poly}). 
To show this, we will first reduce the allocation problem (LP~\ref{eqn:LP}) to a minimum weight $b$-matching problem, which is known to be strongly polynomial \citep{schrijver2003combinatorial}.

Consider an edge-weighted bipartite graph $(N, M, E)$, where $N$ and $M$ are the agent set and set of slots respectively. The set $E$ denotes the edges $(i,j)$ with weights $-v_{ij}$. The matching constraints given by $b_i = 1, \forall i \in N$, and $b_j = k, \forall j \in M$.

\begin{lemma}
\label{lem:equivalence}
 Let $E^* \subseteq E$ be a perfect $b$-matching in $(N, M, E)$ and $A^* = [a_{ij}^*]_{i \in N, j\in M}$ be an allocation where $a_{ij}^* = 1 \Leftrightarrow (i,j) \in E^*$. The matching $E^*$ is a minimum weight perfect $b$-matching iff $A^*$ is an optimal solution to LP~\ref{eqn:LP}.
\end{lemma}

\begin{proof}
 We prove this via contradiction. Suppose $A^*$ is not an optimal solution to LP~\ref{eqn:LP}, i.e., there exists $A'$ which satisfies the constraints and yet gives a larger value to the objective function than that of $A$. Hence, $\sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij}' > \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij}^*$. Consider the edge set $E'$ corresponding to $A'$. Clearly this is a perfect $b$-matching, since $A'$ satisfies the constraints of LP~\ref{eqn:LP}, and $E'$ gives a lower weight than $E^*$, which proves that $E^*$ is not the minimum weight perfect $b$-matching. The implications can be reversed to obtain the other direction of the proof.
\end{proof}
Note that the delays are calculated by solving an equivalent LP like LP~\ref{eqn:LP} with one less agent. Each of these LPs is therefore strongly polynomial and the planner needs to solve $n$ of them. The computation of the each delay needs addition of $2(n-1)$ terms and one subtraction. Hence, the number of computations is polynomial in the number of numbers in the input instance and the space required is polynomial in the size of the input. Therefore we conclude the following.

\begin{corollary}
\label{cor:delay}
 The computation of the delays in \mech\ is strongly polynomial.
\end{corollary}
Combining \Cref{thm:relax}, \Cref{lem:equivalence}, and \Cref{cor:delay},  we get the following result.

\begin{theorem}
 \label{thm:strong}
  \mech\ provides a combinatorial, strongly polynomial algorithm for computing a social schedule and delays.
\end{theorem}

The following section addresses the problem with every agent having jobs with duration spanning multiple time-slots.

\section{Multi-slot Jobs}
\label{sec:multi}

In this section, we consider jobs that has different lengths, i.e., for agent $i$, the job may be of length $l_i \geqslant 1$. In this section, we consider two cases of such jobs, which can be either {\em divisible} or {\em indivisible}. 

\paragraph{Divisible jobs}
In this section, we consider jobs that are {\em divisible}. This means that the job can be broken up into multiple pieces of unit slot-size and can be executed independently within a period. Partial execution of the jobs is also admissible. Examples of such jobs are parallel computer programs with each piece being an independent portion of the code. For social scheduling, these jobs may be completed by an agent via multiple separate visits to the store without any extra cost. The valuation of the job is the sum of the valuations of the allocated slots. We assume that the length $l_i$ of the job is verifiable and is a common knowledge. Hence, the valuations of each of the slots, i.e., $v_{ij}$'s, are the only private information of the agents. In this setting, the valuation of agent $i$ from the allocation $A$ can be written as
\[v_i(A) = \sum_{j : a_{ij} = 1} v_{ij} a_{ij}. \]
Note that the EPP condition under this setting is identical to the IP~\ref{eqn:IP} with the first set of constraints replaced by 
\[ \sum_{j \in M} a_{ij} \leqslant l_i, \ \forall i \in N.\]
Clearly, the LP relaxation of the new IP is identical to LP~\ref{eqn:LP} with the first set of constraints replaced with the above set of constraints. However, this does not alter the constraint matrix $C$, which is TU (shown in the proof of \Cref{thm:relax}). Therefore the new LP also gives integral solutions which is an optimal solution to the new IP. 
The {\em modified} \mech\ is identical to \Cref{algo:mechanism} with Step~\ref{alg:allocation-step} replaced with the solution to the modified LP as explained above.
Hence, the following results hold in a similar manner.

\begin{theorem}
 \label{thm:multi-divisible-dsic}
 Modified \mech\ is per period dominant strategy truthful for multi-slot divisible jobs.
\end{theorem}

\begin{theorem}
 \label{thm:multi-divisible-ir}
 Modified \mech\ is individually rational for every agent.
\end{theorem}

\begin{theorem}
 \label{thm:multi-divisible-relax}
 The allocation of the modified \mech\ always gives integral solutions.
\end{theorem}
Hence, the following corollary also holds.
\begin{corollary}
\label{cor:multi-divisible-efficient}
 Modified \mech\ is EPP.
\end{corollary}
To reduce the allocation problem to a perfect $b$-matching problem, we need to alter $b_i = l_i$, and \Cref{lem:equivalence} holds. Therefore, we conclude that 
\begin{theorem}
 \label{thm:multi-divisible-strong}
  Modified \mech\ provides a combinatorial, strongly polynomial algorithm for computing a social schedule and delays.
\end{theorem}

\paragraph{Indivisible jobs}

A job is {\em indivisible} if the entire length $l_i$ of the job requires contiguous slots for execution within the period. Examples of such jobs are computer programs that are not parallelizable and needs a continuous execution. In the social scheduling setting, an individual may not be willing to visit the store multiple times, and therefore an allocation needs to allocate contiguous time-slots to that agent. We show that the optimal allocation problem in such a setting can be computationally intractable.

To show this, we consider the following simplification of the problem. Agent $i$ comes with a job having a valuation $v_i$ (private) and its length $l_i$ (public). The valuation is independent of the starting point of the job during that period. The value of the job is zero if (a)~it starts at any of the last $l_i - 1$ time-slots of the period (since it cannot finish within the period), and (b)~if the job is unallocated.

A tuple $V$ consists of agents' valuations and $L$ consists of the lengths of agents' jobs. The number of slots within a period are $m$. Each unit of the slot capacity ($k$) can be thought of a counter. Each counter processes one job until it is complete. The set of counters is denoted by $K=\{ 1,2,\dots,k \}$. In this section, we denote the set of all \textit{job-to-counter} allocations by $\mathcal{X}$. An allocation $X\in\mathcal{X}$, is a matrix $[x_{ic}]$ such that:
\begin{equation*}
x_{ic}=
    \begin{cases}
    1, & \text{if agent $i$'s job is allocated to counter $c$}\\
    0, & \text{otherwise}
    \end{cases}
\end{equation*}
\begin{definition}{\textbf{Multi-slot Indivisible Jobs Allocation Problem} (\multi)}: Given $(N,V,L,K,m)$, find $x\in\mathcal{X}$, such that the total valuation of the allocated jobs is maximum subject to the constraints that the total length of jobs allocated to any counter does not exceed the number of slots in that period and each job is assigned to at most one of the counters. Mathematically, \multi\ is given by the following integer program (IP).
\begin{align}
 \label{eqn:MULTIALLOC_IP}
 \begin{split}
     \argmax_{X} & \sum_{c \in K} \sum_{i \in N}   v_{i}\ x_{ic} \\
     \text{s.t. } & \sum_{i \in N} l_i \ x_{ic} \leq m \quad \quad \forall c \in K\\
     & \sum_{c \in K} x_{ic} \leq 1 \quad \quad \forall i \in N\\
     & x_{ic}\in \{ 0,1\} \quad \quad \forall i \in N, \forall c \in K
 \end{split}
\end{align}
\end{definition}
We denote the decision version of \multi\ with the same name which is defined as follows:
\begin{quote} % looks better
Given $(N,V,L,K,m,\beta)$, is there an allocation $X$ such that $\sum_{i \in N} l_i x_{ic} \leqslant m, \ \forall c \in K$, $\sum_{c \in K} x_{ic} \leqslant 1,\  \forall i \in N$, and $\sum_{c \in K} \sum_{i \in N}   v_{i}\ x_{ic}\geqslant \beta$ where $\beta\in\mathbb{R}$.
\end{quote}
\begin{theorem}
\label{thm:NPc}
 \multi\ is NP-complete.
\end{theorem}
\begin{proof} 
% \par $P1$ is a decision problem for the \multi\  implies that, if there exists a polynomial algorithm that solves the $P1$, then one can find the maximum value for the job allocation problem in polynomial time by applying this algorithm iteratively while increasing the value of $b$. On the other hand, if an algorithm finds the optimal value of the job allocation problem in polynomial time, then $P1$ can be solved in polynomial time by comparing the solution output's value by this algorithm the value of $b$. \\
To prove that \multi\  is in $NP$, we have to show that, ``given an allocation $X$, one can verify in polynomial time that $X$ is a valid solution for \multi.'' The verification will need to solve and check the $k+n$ constraints, which are linear inequalities. Therefore, the computation of the value of objective function and comparison with $\beta$ is doable in polynomial time. Hence, \multi\  is in NP.

Next we have to show that, ``every problem in NP is reducible to \multi\  in polynomial time." To prove this, we select the classical \textit{knapsack problem}, which is NP-complete and  show that it is reducible to \multi. The \textit{knapsack problem} is as follows: given a set of items $I=\{1,2,\dots,n\}$, their weights $W=(w_1,w_2,\dots,w_n)$, profits $P=(p_1,p_2,\dots,p_n)$ and a knapsack of capacity $\kappa$, find a subset $Y$ of items from $I$ such that the total profit of the selected items is maximum, and the total weights of the selected items does not exceed $\kappa$. Let $y$ be a vector such that, $y_i=1$ if $i \in Y$, and $y_i=0$ otherwise. The decision version of the knapsack problem is: ``Given $(I,P,W,\kappa,\beta')$, is there a vector $y$ such that $\sum_{i\in I} y_i\ w_i \leq \kappa$, and for which $\sum_{i\in I} p_i y_i \geq$ $\beta'$ where $\beta' \in \mathbb{R}$."

Considering the set of items $I$ as the set of agents $N$, item's profit in $P$ as the value of agent's job in $V$, item's weight in $W$ as the length of the jobs in $L$, and the knapsack with a capacity $\kappa$ as the single counter available till $\kappa$ number of slots; the knapsack problem $(I,P,W,\kappa,\beta')$ is reducible in polynomial time to \multi\ $(I,P,W,\{1\},\kappa, \beta')$.
\end{proof}

Our primary objective in this paper is to find a computationally tractable mechanism that satisfies the desired properties outlined in \Cref{sec:desiderata}. We see that in the context of indivisible job allocation, the problem of finding the efficient allocation is intractable. However, it may be possible to find an approximately efficient tractable allocation which is truthful and individually rational. We leave this problem for a future investigation.

In the following section, we investigate the performance of \mech\ in real-world scenarios.


==> preamble_oth.tex <==
\newcommand{\qedb}{\hfill\ensuremath{\blacksquare}}

% %%% MY HEADER
% \renewcommand{\baselinestretch}{1.0}
% \usepackage{fullpage}
% \usepackage{xcolor}
% \usepackage[switch]{lineno}
% \linenumbers
\usepackage{wrapfig}
% \usepackage{ae,aecompl}
%\usepackage{doublespace}
% \usepackage[dvips]{graphicx}
\usepackage{amssymb}
\usepackage{amsmath}
%%% To reduce the gap between equations
%\g@addto@macro\normalsize{%
%  \setlength\abovedisplayskip{5pt}
%  \setlength\belowdisplayskip{5pt}
%  \setlength\abovedisplayshortskip{5pt}
%  \setlength\belowdisplayshortskip{5pt}
%}

% \usepackage{wrapfig}
% \usepackage{subfigure}
\usepackage{subcaption}
\usepackage{framed}
\usepackage{footmisc}
% \usepackage{authblk}
\usepackage[round,authoryear]{natbib}
% \usepackage[square, comma, sort&compress]{natbib}
% \citestyle{authordate}
% \usepackage{epsf}
% \usepackage{color}
% \usepackage{array}
\usepackage{authblk}
%\usepackage{rotating}
\usepackage{colortbl}
\definecolor{webgreen}{rgb}{0,0.4,0}
\definecolor{webbrown}{rgb}{0.6,0,0}
\definecolor{purple}{rgb}{0.5,0,0.25}
\definecolor{darkblue}{rgb}{0,0,0.7}
\definecolor{darkred}{rgb}{0.7,0,0}
%\usepackage{html}
%\usepackage{times}
%\usepackage[dvips,pdfborder=false]{hyperref}
\usepackage{hyperref}
\hypersetup{colorlinks,citecolor=darkblue,filecolor=black,linkcolor=darkred,urlcolor=webgreen,pdfpagemode=None,
pdfstartview=FitH}

\newcommand{\ignore}[1]{}
\newcommand{\score}{{\tt sc}}
\newcommand{\estscore}{\hat{\tt sc}}
\newcommand{\estnum}{\hat{N}}
\newcommand{\estp}{\hat{p}}
\newcommand{\estq}{\hat{q}}
\newcommand{\beat}{\text{Beat}}
\newcommand{\nbr}{\text{Nbr}}
\newcommand{\given}{\ | \ }
\newcommand{\whp}{\textit{w.h.p}}
\newcommand{\surp}{{\tt surp}}
\newcommand{\mpfb}{{\tt MPFB}}


% % Voting rules
\newcommand{\plu}{{\tt Plu}}
\newcommand{\bor}{{\tt Bor}}
\newcommand{\veto}{{\tt Vet}}
\newcommand{\cope}{{\tt Cop}}

% \renewenvironment{abstract}{\begin{abstract}\noindent\ignorespaces}{\end{abstract}}
% \usepackage{etoolbox}
% \ifundef{\abstract}{}{\patchcmd{\abstract}%
%     {\quotation}{\quotation\noindent\ignorespaces}{}{}}

\usepackage{amsthm}
% %%% this is to restate a theorem
% \makeatletter
% \newtheorem*{rep@theorem}{\rep@title}
% \newcommand{\newreptheorem}[2]{%
% \newenvironment{rep#1}[1]{%
%  \def\rep@title{#2 \ref{##1}}%
%  \begin{rep@theorem}}%
%  {\end{rep@theorem}}}
% \makeatother
% %%% this is to restate a theorem

\newtheorem{lemma}{{\sc Lemma}}
\newtheorem{proposition}{{\sc Proposition}}
\newtheorem{corollary}{{\sc Corollary}}
\newtheorem{theorem}{{\sc Theorem}}
\newtheorem{definition}{{\sc Definition}}
\newtheorem{observation}{{\sc Observation}}
\newtheorem{claim}{{\sc Claim}}
\newtheorem{example}{{\sc Example}}
\newtheorem{discussion}{{\sc Discussion}}
\newtheorem{mechanism}{{\sc Mechanism}}
\newtheorem{question}{{\sc Question}}
\newtheorem{fact}{{\sc Fact}}
\newtheorem{assumption}{{\sc Assumption}}
% \newreptheorem{fact}{{\sc Fact}}

\sloppy
\usepackage{cleveref}
\crefname{claim}{claim}{claims}
\crefname{fact}{fact}{facts}
\crefname{algorithm}{algorithm}{algorithms}
\crefname{observation}{observation}{observations}
\crefname{equation}{equation}{equations}
\crefname{assumption}{assumption}{assumptions}

% \newenvironment{proof}{\noindent {\em Proof\/}:\enspace}
% {\hfill $\blacksquare{}$ \medskip \\}
\newenvironment{psketch}{\noindent {\em Proof sketch\/}:\enspace}
{\hfill $\blacksquare{}$ \medskip \\}
\newenvironment{proof1}[1]{\noindent {\em Proof\/} (#1):\enspace}
{\hfill $\blacksquare{}$ \medskip \\}
\newcommand{\sectitle}[1]{\large \bf \sf#1}


% %%% Swaprava's new title
% \usepackage{titlesec}
% 
% \titlespacing*{\section}{0pt}{6pt plus 2pt minus 2pt}{6pt plus 2pt minus 2pt}
% \titlespacing*{\subsection}{0pt}{6pt plus 2pt minus 2pt}{6pt plus 2pt minus 2pt}
% \titlespacing*{\subsubsection}{0pt}{6pt plus 2pt minus 2pt}{6pt plus 2pt minus 2pt}


\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\diag}{\mathrm{diag}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\sw}{\text{\tt sw}}
\newcommand{\q}[1]  {\noindent \textcolor{red}{{\bf Question: }{\em #1?}}}

% \newcommand\xleftrightarrow[2][]{%
%   \ext@arrow 9999{\longleftrightarrowfill@}{#1}{#2}}
% \newcommand\longleftrightarrowfill@{%
%   \arrowfill@\leftarrow\relbar\rightarrow}
%%%

% \usepackage{hyperref}
\usepackage{pgf}
\usepackage{mathtools}
% \usepackage{tikz}
% \usepackage{varwidth}
% \usetikzlibrary{shapes,arrows, trees}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}

% \usepackage{multirow,bigdelim}
% \usepackage{arydshln}
\usepackage{resizegather}
% \usepackage[noend]{algpseudocode}
% \sloppy
% \usepackage{cleveref}
% \crefname{fact}{fact}{facts}
% \crefname{algorithm}{algorithm}{algorithms}

\newcommand{\gs}[1]  {\noindent \textcolor{brown}{{\bf GS: }{``\em #1''}}}

% Swaprava: here I declare the environment for editing. To include the edit in the final text, just remove \snedit{text} to text
\newcommand{\sn}[1]  {\noindent \textcolor{blue}{{\bf SN: }{``\em #1''}}}
% \newcommand{\test}[2]  {\noindent \textcolor{blue}{{\bf SN: }{``\em #1''}} {\textcolor{red}{#2}}}
% \DeclareMathAlphabet{\mathscr}{OT1}{pzc}{m}{it}
% \newcommand{\snedit}[1]  {{\textcolor{blue}{ #1}}}


%Palash: changes begin
%changing font
% \usepackage[T1]{fontenc}
% \usepackage{charter,eulervm}
\usepackage{url}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\renewcommand{\labelitemi}{$\vartriangleright$}

\usepackage{xspace}
\newcommand{\el}{\ensuremath{\ell}\xspace}
\newcommand{\suc}{\ensuremath{\succ}\xspace}
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\pr}{\prime\xspace}
\newcommand{\Nvec}{\vec{N}}

\newcommand{\EB}{\ensuremath{\mathbb E}\xspace}
\newcommand{\PB}{\ensuremath{\mathbb P}\xspace}
\newcommand{\RB}{\ensuremath{\mathbb R}\xspace}

\renewcommand{\AA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\BB}{\ensuremath{\mathcal B}\xspace}
\newcommand{\CC}{\ensuremath{\mathcal C}\xspace}
\newcommand{\DD}{\ensuremath{\mathcal D}\xspace}
\newcommand{\EE}{\ensuremath{\mathcal E}\xspace}
\newcommand{\FF}{\ensuremath{\mathcal F}\xspace}
\newcommand{\GG}{\ensuremath{\mathcal G}\xspace}
\newcommand{\HH}{\ensuremath{\mathcal H}\xspace}
\newcommand{\II}{\ensuremath{\mathcal I}\xspace}
\newcommand{\JJ}{\ensuremath{\mathcal J}\xspace}
\newcommand{\KK}{\ensuremath{\mathcal K}\xspace}
\newcommand{\LL}{\ensuremath{\mathcal L}\xspace}
\newcommand{\MM}{\ensuremath{\mathcal M}\xspace}
\newcommand{\NN}{\ensuremath{\mathcal N}\xspace}
\newcommand{\OO}{\ensuremath{\mathcal O}\xspace}
\newcommand{\PP}{\ensuremath{\mathcal P}\xspace}
\newcommand{\QQ}{\ensuremath{\mathcal Q}\xspace}
\newcommand{\RR}{\ensuremath{\mathcal R}\xspace}
\renewcommand{\SS}{\ensuremath{\mathcal S}\xspace}
\newcommand{\TT}{\ensuremath{\mathcal T}\xspace}
\newcommand{\UU}{\ensuremath{\mathcal U}\xspace}
\newcommand{\VV}{\ensuremath{\mathcal V}\xspace}
\newcommand{\WW}{\ensuremath{\mathcal W}\xspace}
\newcommand{\XX}{\ensuremath{\mathcal X}\xspace}
\newcommand{\YY}{\ensuremath{\mathcal Y}\xspace}
\newcommand{\ZZ}{\ensuremath{\mathcal Z}\xspace}

\newcommand{\aaa}{\ensuremath{\mathfrak a}\xspace}
\newcommand{\bbb}{\ensuremath{\mathfrak b}\xspace}
\newcommand{\ccc}{\ensuremath{\mathfrak c}\xspace}
\newcommand{\ddd}{\ensuremath{\mathfrak d}\xspace}
\newcommand{\eee}{\ensuremath{\mathfrak e}\xspace}
\newcommand{\fff}{\ensuremath{\mathfrak f}\xspace}
\renewcommand{\ggg}{\ensuremath{\mathfrak g}\xspace}
\newcommand{\hhh}{\ensuremath{\mathfrak h}\xspace}
\newcommand{\iii}{\ensuremath{\mathfrak i}\xspace}
\newcommand{\jjj}{\ensuremath{\mathfrak j}\xspace}
\newcommand{\kkk}{\ensuremath{\mathfrak k}\xspace}
\renewcommand{\lll}{\ensuremath{\mathfrak f}\xspace}
\newcommand{\mmm}{\ensuremath{\mathfrak m}\xspace}
\newcommand{\nnn}{\ensuremath{\mathfrak n}\xspace}
\newcommand{\ooo}{\ensuremath{\mathfrak o}\xspace}
\newcommand{\ppp}{\ensuremath{\mathfrak p}\xspace}
\newcommand{\qqq}{\ensuremath{\mathfrak q}\xspace}
\newcommand{\rrr}{\ensuremath{\mathfrak r}\xspace}
\newcommand{\sss}{\ensuremath{\mathfrak s}\xspace}
\newcommand{\ttt}{\ensuremath{\mathfrak t}\xspace}
\newcommand{\uuu}{\ensuremath{\mathfrak u}\xspace}
\newcommand{\vvv}{\ensuremath{\mathfrak v}\xspace}
\newcommand{\www}{\ensuremath{\mathfrak w}\xspace}
\newcommand{\xxx}{\ensuremath{\mathfrak x}\xspace}
\newcommand{\yyy}{\ensuremath{\mathfrak y}\xspace}
\newcommand{\zzz}{\ensuremath{\mathfrak z}\xspace}

\usepackage{nicefrac}
\newcommand{\ffrac}{\flatfrac}
\newcommand{\nfrac}{\nicefrac}

\usepackage{enumitem}
\usepackage{multirow}

\usepackage{dsfont}

\newcounter{casenum}
\newenvironment{caseof}{\setcounter{casenum}{1}}{\vskip.5\baselineskip}
\newcommand{\case}[2]{\vskip.5\baselineskip\par\noindent {\bfseries Case \arabic{casenum}:} #1\\#2\addtocounter{casenum}{1}}





